Every Sequence is Decompressible from a Random One

Kucera and Gacs independently showed that every infinite sequence is Turing reducible to a Martin-Lof random sequence. This result is extended by showing that every infinite sequence S is Turing reducible to a Martin-Lof random sequence R such that the asymptotic number of bits of R needed to compute n bits of S, divided by n, is precisely the constructive dimension of S. It is shown that this is the optimal ratio of query bits to computed bits achievable with Turing reductions. As an application of this result, a new characterization of constructive dimension is given in terms of Turing reduction compression ratios.

==> bigpage.tex <==
% This is a file needed to make the pages not look like ass after going 
% through CoRR's automatic compilation that normally destroys margins.

\oddsidemargin  0.0in
\evensidemargin 0.0in
\textwidth      6.3in
\headheight     0.0in
\topmargin      -0.3in
\textheight     8.7in


